Pull Request Latency Explained: An Empirical Overview

Pull request latency evaluation is an essential application of effort evaluation in the pull-based development scenario. It can help the reviewers sort the pull request queue, remind developers about the review processing time, speed up the review process and accelerate software development. There is a lack of work that systematically organizes the factors that affect pull request latency. Also, there is no related work discussing the differences and variations in characteristics in different scenarios and contexts. In this paper, we collected relevant factors through a literature review approach. Then we assessed their relative importance in five scenarios and six different contexts using the mixed-effects linear regression model. We find that the relative importance of factors differs in different scenarios, e.g., the first response time of the reviewer is most important when there exist comments. Meanwhile, the number of commits in a pull request has a more significant impact on pull request latency when closing than submitting due to changes in contributions brought about by the review process.

==> tables/factors_correlation.tex <==
%!TEX root = ../main.tex
\begin{table}[htbp]
    \centering
    \caption{Choices and corresponding reasons for strongly correlated factors}
    \label{strongly_correlated_factors}
    \begin{tabular}{ p{3cm} p{2.5cm} p{1.8cm} }
      \toprule
      \textbf{Correlated factors} & \textbf{Selected factor} & \textbf{Reason} \\ \hline
      
      test\_lines\_per\_kloc & \multirow{3}{*}{\emph{test\_lines\_per\_kloc}} & \multirow{3}{*}{previous study}\\
      test\_cases\_per\_kloc & & \\
      asserts\_per\_kloc & &  \\ \hdashline
      
      src\_churn & \multirow{3}{*}{\emph{src\_churn}} & \multirow{3}{*}{frequency} \\
      churn\_addition & & \\
      churn\_deletion & & \\ \hdashline
    
      num\_comments & \multirow{4}{*}{\emph{num\_comments}} & \multirow{4}{*}{frequency} \\
      at\_tag & & \\
      num\_participants & & \\
      num\_comments\_con & & \\ \hdashline
      
      core\_member & \multirow{4}{*}{\emph{core\_member}} & \multirow{4}{*}{frequency} \\
      perc\_external\_contribs & & \\
      social\_strength & & \\
      requester\_succ\_rate & & \\ \hdashline
      
      stars & \multirow{3}{*}{\emph{stars}} & \multirow{3}{*}{frequency} \\
      fork\_num & & \\
      inte\_affiliation & & \\ \hdashline
      
      prev\_pullreqs & \multirow{2}{*}{\emph{prev\_pullreqs}} & \multirow{2}{*}{frequency} \\
      prior\_interaction & \\ \hdashline
      
      num\_code\_comments & \multirow{3}{*}{\emph{num\_code\_comments}} & \multirow{3}{*}{frequency} \\
      part\_num\_code & & \\
      num\_code\_comments\_con & & \\ \hdashline
      
      open\_pr\_num & \multirow{2}{*}{\emph{open\_pr\_num}} & \multirow{2}{*}{frequency} \\
      fork\_num & \\ \hdashline
    
      ci\_latency & \multirow{2}{*}{\emph{ci\_latency}} & \multirow{2}{*}{importance} \\
      ci\_build\_num & & \\ \hdashline
    
      sloc & \multirow{2}{*}{\emph{sloc}} & \multirow{2}{*}{importance} \\
      language & & \\ \hdashline
    
      has\_comments & \multirow{6}{*}{\emph{has\_comments}} & \multirow{6}{*}{expressiveness} \\
      has\_participants & & \\ 
      core\_comment & & \\
      contrib\_comment & & \\
      inte\_comment & & \\
      has\_exchange & & \\ \hdashline
      
      prior\_review\_num & \multirow{2}{*}{\emph{prior\_review\_num}} & \multirow{2}{*}{data availability} \\
      inte\_affiliation & \\ \hdashline
    
      open\_issue\_num & \multirow{2}{*}{\emph{open\_issue\_num}} & \multirow{2}{*}{data availability} \\ 
      inte\_affiliation & \\ \hdashline
      
      inte\_cons & \multirow{2}{*}{\emph{inte\_cons}} & \multirow{2}{*}{data availability} \\
      inte\_affiliation & \\ \hdashline
      
      inte\_extra & \multirow{2}{*}{\emph{inte\_extra}} & \multirow{2}{*}{data availability} \\
      inte\_affiliation & \\ \hdashline
      
      inte\_agree & \multirow{2}{*}{\emph{inte\_agree}} & \multirow{2}{*}{data availability} \\
      inte\_affiliation & \\ \hdashline
    
      same\_country & \multirow{2}{*}{\emph{same\_country}} & \multirow{2}{*}{discussion} \\
      contrib\_country & & \\ \hdashline
      
      perc\_contrib\_pos\_emo & \multirow{2}{*}{\emph{perc\_contrib\_pos\_emo}} & \multirow{2}{*}{discussion} \\
      contrib\_first\_emo & \\ \hdashline
      
      perc\_inte\_neg\_emo & \multirow{2}{*}{\emph{perc\_inte\_neg\_emo}} & \multirow{2}{*}{discussion} \\
      inte\_first\_emo & & \\ \hdashline
      
      perc\_inte\_pos\_emo & \multirow{2}{*}{\emph{perc\_inte\_pos\_emo}} & \multirow{2}{*}{discussion} \\
      inte\_first\_emo & & \\ \hdashline
      
      same\_user & \multirow{5}{*}{\emph{same\_user}} & \multirow{5}{*}{discussion} \\
      inte\_first\_emo & \\ 
      inte\_affiliation & \\
      contrib\_affiliation & \\ 
      contrib\_rate\_author & \\ \hdashline
    
      same\_affiliation & \multirow{2}{*}{\emph{same\_affiliation}} & \multirow{2}{*}{discussion} \\
      contrib\_affiliation & & \\ \hdashline
    
      perc\_neg\_emotion & \multirow{4}{*}{\emph{perc\_neg\_emotion}} & \multirow{4}{*}{discussion} \\
      perc\_contrib\_neg\_emo & & \\
      contrib\_first\_emo & & \\
      inte\_first\_emo & & \\ \hdashline
      
      perc\_pos\_emotion & \multirow{2}{*}{\emph{perc\_pos\_emotion}} & \multirow{2}{*}{discussion} \\
      inte\_first\_emo & & \\ \hdashline
    
      ci\_failed\_perc & \multirow{4}{*}{\emph{ci\_failed\_perc}} & \multirow{4}{*}{discussion} \\
      ci\_test\_passed & & \\
      ci\_first\_build\_status & & \\
      ci\_last\_build\_status & & \\ \bottomrule
      
    \end{tabular}
    \end{table}
    

==> tables/results_RQ2_2-before-2021-08-05.tex <==
% Table generated by Excel2LaTeX from sheet 'RQ2_2'
% for open_pr_num and ci_exists contexts
\clearpage
\setlength{\rotFPtop}{0pt plus 1fil}
\begin{sidewaystable*}
    % \centering
    \setlength{\tabcolsep}{0.2em}
    \tiny
    \renewcommand{\arraystretch}{1.25}
    \caption{Results for comparing factors influencing pull request latency in different contexts. - means the factor is not included in the model. Red color marks the factors with at least 5\% of variance change across different contexts.}
    \label{table:results_RQ2_2}
    \begin{tabular}{clr@{(}l@{)}lr@{.}llr@{(}l@{)}lr@{.}llr@{(}l@{)}lr@{.}llr@{(}l@{)}lr@{.}llr@{(}l@{)}lr@{.}ll}
        \toprule
        & \multicolumn{1}{c}{(1)} & \multicolumn{3}{c}{(2)} & \multicolumn{3}{c}{(3)} & \multicolumn{3}{c}{(4)} & \multicolumn{3}{c}{(5)} & \multicolumn{3}{c}{(6)} & \multicolumn{3}{c}{(7)} & \multicolumn{3}{c}{(8)} & \multicolumn{3}{c}{(9)} & \multicolumn{3}{c}{(10)} & \multicolumn{3}{c}{(11)} \\
        \cmidrule(r){2-32}
        & & \multicolumn{18}{c}{\textbf{\emph{Project context}}} & \multicolumn{12}{c}{\textbf{\emph{Tool context}}} \\
        \cmidrule(r){3-20} \cmidrule(r){21-32}
        & & \multicolumn{6}{c}{\textbf{\emph{$open\_pr\_num \leq6$}}} & \multicolumn{6}{c}{\textbf{\emph{$6<open\_pr\_num \leq29$}}} & \multicolumn{6}{c}{\textbf{\emph{$open\_pr\_num >29$}}} & \multicolumn{6}{c}{\textbf{\emph{ci\_exists=1}}} & \multicolumn{6}{c}{\textbf{\emph{ci\_exists=0}}} \\
        \cmidrule(r){3-8} \cmidrule(r){9-14} \cmidrule(r){15-20} \cmidrule(r){21-26} \cmidrule(r){27-32}

        & & \multicolumn{3}{c}{Coeffs (Err.)} & \multicolumn{3}{c}{Sum sq} & \multicolumn{3}{c}{Coeffs (Err.)} & \multicolumn{3}{c}{Sum sq} & \multicolumn{3}{c}{Coeffs (Err.)} & \multicolumn{3}{c}{Sum sq} & \multicolumn{3}{c}{Coeffs (Err.)} & \multicolumn{3}{c}{Sum sq} & \multicolumn{3}{c}{Coeffs (Err.)} & \multicolumn{3}{c}{Sum sq} \\
        \cmidrule(r){2-32}
        
        (1)   &  (Intercept) & -0.37  & 0.01  & ***   & \multicolumn{3}{c}{}  & -0.46  & 0.01  & ***   & \multicolumn{3}{c}{}  & -0.59  & 0.01  & ***   & \multicolumn{3}{c}{}  & -0.40  & 0.01  & ***   & \multicolumn{3}{c}{}  & -0.43  & 0.01  & ***   & \multicolumn{3}{c}{} \\
        (2)   &  has\_comments & 0.47  & 0.00  & ***   & 23693 & 30    & ***   & 0.49  & 0.00  & ***   & 27369 & 27    & ***   & 0.48  & 0.00  & ***   & 30315 & 46    & ***   & 0.46  & 0.00  & ***   & 60777 & 88    & ***   & 0.51  & 0.00  & ***   & 19134 & 56    & *** \\
        (3)   &  same\_user0 & \textcolor{red}{0.37} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{12838} & \textcolor{red}{83} & \textcolor{red}{***} & \textcolor{red}{0.34} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{11351} & \textcolor{red}{86} & \textcolor{red}{***} & \textcolor{red}{0.30} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{10687} & \textcolor{red}{50} & \textcolor{red}{***} & \textcolor{red}{0.31} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{23586} & \textcolor{red}{66} & \textcolor{red}{***} & \textcolor{red}{0.42} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{11974} & \textcolor{red}{70} & \textcolor{red}{***} \\
        (4)   &  description\_length & 0.13  & 0.00  & ***   & 8067  & 56    & ***   & 0.13  & 0.00  & ***   & 8316  & 96    & ***   & 0.13  & 0.00  & ***   & 10774 & 34    & ***   & 0.13  & 0.00  & ***   & 19837 & 71    & ***   & 0.14  & 0.00  & ***   & 6071  & 56    & *** \\
        (5)   &  \makecell[l]{num\_commits\_\\close} & 0.12  & 0.00  & ***   & 4814  & 66    & ***   & 0.11  & 0.00  & ***   & 3834  & 64    & ***   & 0.10  & 0.00  & ***   & 3760  & 20    & ***   & 0.12  & 0.00  & ***   & 12085 & 98    & ***   & 0.08  & 0.00  & ***   & 1342  & 72    & *** \\
        (6)   &  num\_code\_comments & \textcolor{red}{0.08} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{3087} & \textcolor{red}{16} & \textcolor{red}{***} & \textcolor{red}{0.10} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{4995} & \textcolor{red}{38} & \textcolor{red}{***} & \textcolor{red}{0.14} & \textcolor{red}{0.00} & \textcolor{red}{***} & \textcolor{red}{11898} & \textcolor{red}{00} & \textcolor{red}{***} & 0.12  & 0.00  & ***   & 16251 & 90    & ***   & 0.09  & 0.00  & ***   & 2552  & 44    & *** \\
        (7)   &  integrator\_availability & 0.07  & 0.00  & ***   & 2883  & 75    & ***   & 0.07  & 0.00  & ***   & 3137  & 27    & ***   & 0.06  & 0.00  & ***   & 2481  & 84    & ***   & 0.07  & 0.00  & ***   & 6846  & 15    & ***   & 0.07  & 0.00  & ***   & 1782  & 75    & *** \\
        (8)   &  hash\_tag1 & 0.15  & 0.00  & ***   & 1705  & 40    & ***   & 0.16  & 0.00  & ***   & 2662  & 82    & ***   & 0.15  & 0.00  & ***   & 3218  & 66    & ***   & 0.16  & 0.00  & ***   & 7148  & 17    & ***   & 0.12  & 0.00  & ***   & 680   & 55    & *** \\
        (9)   &  \makecell[l]{src\_churn\_\\close} & 0.07  & 0.00  & ***   & 1565  & 15    & ***   & 0.08  & 0.00  & ***   & 2281  & 88    & ***   & 0.10  & 0.00  & ***   & 3841  & 85    & ***   & 0.09  & 0.00  & ***   & 6598  & 17    & ***   & 0.07  & 0.00  & ***   & 1035  & 85    & *** \\
        (10)  &  open\_pr\_num & 0.06  & 0.00  & ***   & 1340  & 24    & ***   & 0.06  & 0.00  & ***   & 1015  & 30    & ***   & 0.17  & 0.00  & ***   & 1635  & 55    & ***   & 0.19  & 0.00  & ***   & 5479  & 78    & ***   & 0.12  & 0.00  & ***   & 855   & 65    & *** \\
        (11)  &  core\_member1 & -0.13  & 0.00  & ***   & 1054  & 35    & ***   & -0.11  & 0.00  & ***   & 635   & 93    & ***   & -0.05  & 0.00  & ***   & 147   & 83    & ***   & -0.08 & 0.00  & ***   & 907   & 11    & ***   & -0.14  & 0.00  & ***   & 889   & 73    & *** \\
        (12)  &  ci\_exists1 & 0.10  & 0.00  & ***   & 505   & 51    & ***   & 0.13  & 0.00  & ***   & 683   & 65    & ***   & 0.14  & 0.00  & ***   & 898   & 79    & ***   & \multicolumn{12}{c}{-} \\
        (13)  &  prev\_pullreqs & -0.05  & 0.00  & ***   & 453   & 47    & ***   & -0.04  & 0.00  & ***   & 372   & 18    & ***   & -0.08  & 0.00  & ***   & 1649  & 82    & ***   & -0.06 & 0.00  & ***   & 1981  & 65    & ***   & -0.05  & 0.00  & ***   & 404   & 70    & *** \\
        (14)  &  project\_age & 0.05  & 0.00  & ***   & 451   & 25    & ***   & -0.02  & 0.00  & ***   & 39    & 67    & ***   & -0.05  & 0.00  & ***   & 386   & 52    & ***   & 0.02  & 0.00  & ***   & 187   & 82    & ***   & 0.02  & 0.00  & ***   & 29    & 78    & *** \\
        (15)  &  reopen\_or\_not1 & 0.22  & 0.01  & ***   & 361   & 58    & ***   & 0.25  & 0.01  & ***   & 549   & 11    & ***   & 0.31  & 0.01  & ***   & 1599  & 75    & ***   & 0.28  & 0.00  & ***   & 2188  & 86    & ***   & 0.21  & 0.01  & ***   & 248   & 20    & *** \\
        (16)  &  \makecell[l]{commits\_on\_files\_\\touched\_close} & -0.03  & 0.00  & ***   & 283   & 88    & ***   & -0.03  & 0.00  & ***   & 428   & 99    & ***   & -0.03  & 0.00  & ***   & 472   & 66    & ***   & -0.03 & 0.00  & ***   & 1160  & 42    & ***   & -0.03  & 0.00  & ***   & 213   & 24    & *** \\
        (17)  &  friday\_effect1 & 0.04  & 0.00  & ***   & 182   & 66    & ***   & 0.06  & 0.00  & ***   & 320   & 15    & ***   & 0.06  & 0.00  & ***   & 439   & 41    & ***   & 0.06  & 0.00  & ***   & 859   & 80    & ***   & 0.04  & 0.00  & ***   & 90    & 20    & *** \\
        (18)  &  \makecell[l]{test\_churn\_\\close} & 0.02  & 0.00  & ***   & 126   & 26    & ***   & 0.02  & 0.00  & ***   & 125   & 85    & ***   & 0.03  & 0.00  & ***   & 238   & 26    & ***   & 0.02  & 0.00  & ***   & 375   & 95    & ***   & 0.01  & 0.00  & ***   & 39    & 84    & *** \\
        (19)  &  prior\_review\_num & 0.02  & 0.00  & ***   & 94    & 13    & ***   & 0.02  & 0.00  & ***   & 205   & 57    & ***   & 0.01  & 0.00  & ***   & 36    & 60    & ***   & 0.01  & 0.00  & ***   & 180   & 30    & ***   & 0.00  & 0.00  & **    & 4     & 52    & ** \\
        (20)  & followers & -0.01  & 0.00  & ***   & 34    & 45    & ***   & -0.01  & 0.00  & ***   & 50    & 11    & ***   & 0.00  & 0.00  & ***   & 8     & 71    & ***   & -0.01  & 0.00  & ***   & 76    & 38    & ***   & -0.01  & 0.00  & ***   & 8     & 77    & *** \\
        (21)  &  sloc & -0.01  & 0.00  & ***   & 7     & 88    & ***   & -0.01  & 0.00  & ***   & 10    & 52    & ***   & -0.05  & 0.00  & ***   & 157   & 63    & ***   & -0.02  & 0.00  & ***   & 44    & 57    & ***   & 0.00  & 0.00  &       & 0     & 81    &  \\
        (22)  &  \makecell[l]{files\_changed\_\\close} & -0.01  & 0.00  & ***   & 7     & 29    & ***   & 0.00  & 0.00  & *     & 3     & 80    & *     & -0.03  & 0.00  & ***   & 260   & 27    & ***   & -0.01  & 0.00  & ***   & 98    & 66    & ***   & 0.00  & 0.00  & .     & 1     & 78    & . \\
        (23)  &  contrib\_genderMale & 0.01  & 0.00  & *     & 3     & 16    & *     & 0.01  & 0.00  &       & 1     & 58    &       & 0.01  & 0.00  & ***   & 9     & 19    & ***   & 0.01  & 0.00  & ***   & 19    & 63    & ***   & 0.00  & 0.00  &       & 0     & 60    &  \\
        (24)  &  test\_lines\_per\_kloc & 0.01  & 0.00  & *     & 3     & 14    & *     & -0.02  & 0.00  & ***   & 20    & 15    & ***   & 0.01  & 0.00  & *     & 2     & 79    & *     & 0.00  & 0.00  &       & 0     & 39    &       & -0.01  & 0.00  & *     & 2     & 83    & * \\
        (25)  &  \makecell[l]{test\_inclusion\_\\close1} & 0.01  & 0.00  & *     & 2     & 40    & *     & 0.00  & 0.00  &       & 0     & 51    &       & 0.01  & 0.00  & **    & 4     & 78    & **    & 0.00  & 0.00  & *     & 2     & 53    & *     & 0.01  & 0.00  & .     & 1     & 82    & . \\
        (26)  &  team\_size & 0.00  & 0.00  &       & 0     & 70    &       & -0.03  & 0.00  & ***   & 123   & 54    & ***   & -0.09  & 0.00  & ***   & 743   & 10    & ***   & -0.04  & 0.00  & ***   & 288   & 42    & ***   & -0.03  & 0.00  & ***   & 52    & 82    & *** \\


        \cmidrule(r){1-32}
        &  nobs & \multicolumn{6}{c}{744,796}                    & \multicolumn{6}{c}{771,009}                    & \multicolumn{6}{c}{897,634}                    & \multicolumn{6}{c}{1,885,836}                   & \multicolumn{6}{c}{527,603} \\
        &  $R^{2}_m$  & \multicolumn{6}{c}{0.32}                      & \multicolumn{6}{c}{0.3}                       & \multicolumn{6}{c}{0.3}                       & \multicolumn{6}{c}{0.32}                      & \multicolumn{6}{c}{0.34} \\
        &  $R^{2}_c$  & \multicolumn{6}{c}{0.44}                      & \multicolumn{6}{c}{0.42}                      & \multicolumn{6}{c}{0.41}                      & \multicolumn{6}{c}{0.42}                      & \multicolumn{6}{c}{0.48} \\
        \bottomrule
    \end{tabular}%
\end{sidewaystable*}
\clearpage
